CFG-Zero*: Improved Classifier-Free Guidance for Flow Matching Models

Classifier-Free Guidance (CFG) is a widely adopted technique in diffusion/flow models to improve image fidelity and controllability. In this work, we first analytically study the effect of CFG on flow matching models trained on Gaussian mixtures where the ground-truth flow can be derived. We observe that in the early stages of training, when the flow estimation is inaccurate, CFG directs samples toward incorrect trajectories. Building on this observation, we propose CFG-Zero*, an improved CFG with two contributions: (a) optimized scale, where a scalar is optimized to correct for the inaccuracies in the estimated velocity, hence the * in the name; and (b) zero-init, which involves zeroing out the first few steps of the ODE solver. Experiments on both text-to-image (Lumina-Next, Stable Diffusion 3, and Flux) and text-to-video (Wan-2.1) generation demonstrate that CFG-Zero* consistently outperforms CFG, highlighting its effectiveness in guiding Flow Matching models. (Code is available at github.com/WeichenFan/CFG-Zero-star)

==> figs/teaser.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{assets/teaser_dist.pdf}
\caption{\textbf{The sampling trajectory on synthetic mixed Gaussian in $\sR^2$.} The gray dashed line denotes the optimal trajectory from $x_0$ to $x_1$, where \ours denoted in \textcolor{ForestGreen}{green} line is more accurate compared to CFG in \textcolor{orange}{orange} line. \yijia{Do we show \ours here?}
}
\label{fig:teaser}
\end{figure}

% \begin{center}
%     \captionsetup{type=figure}
%     %\vspace{-19pt}
%     \includegraphics[width=1.0\linewidth]{assets/teaser_figure.pdf}
%     %\vspace{-20pt}
%     \captionof{figure}{xxx}
%     \label{fig:demo_dia}
% \end{center}

==> src/discuss.tex <==
\section{Discussion}
\ray{TODO: I don't think we need this.}
This work introduces a novel perspective to improve the classifier-free guidance in flow-matching based models. However, we only explore the our method within the flow-matching based models. Moving forward, we envision future research directions focusing on further optimizing guidance dynamics in score-based models, exploring adaptive learning strategies for eliminating the error induced by the unwell-trained conditional and unconditional models. As for the broader impact, generative models offer powerful capabilities but also pose risks, including misinformation and misuse for deceptive purposes. We hope this work contributes to a better understanding of these models, helping to develop strategies that mitigate potential harms while advancing responsible AI development.

==> tabs/user.tex <==
\begin{table}[t]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{l c c c c c}
\toprule
Model & Overall Score$\uparrow$ & Detail Score$\uparrow$ & Color$\uparrow$ & Image-Text Alignment$\uparrow$\\
\midrule
Lumina~\cite{luminanext} & 71.02\% & 70.45\% & 71.24\% & 52.35\% \\

SD3~\cite{sd3} & 71.22\% & 70.48\% & 71.72\% & 53.23\% \\

SD3.5~\cite{sd3} & 72.15\% & 82.33\% & 81.45\% & 53.33\% \\

Flux~\cite{flux} & 55.72\% & 70.15\% & 65.13\% & 55.74\% \\
\bottomrule
\end{tabular}}
\caption{\textbf{User study on Lumina-Next, Stable Diffusion 3, Stable Diffusion 3.5, and Flux}. The win rate of our method compared to CFG is presented.\textcolor{red}{TODO: change to Fig}}
\label{tab:user}
\end{table}
